Explaining the Entombed Algorithm

In \cite{entombed}, John Aycock and Tara Copplestone pose an open question, namely the explanation of the mysterious lookup table used in the Entombed Game's Algorithm for two dimensional maze generation. The question attracted media attention (BBC etc) and was open until today. This paper answers this question, explains the algorithm and even extends it to three dimensions.

==> env.tex <==
\subsection{Implementing $\texttt{Solve}_{x,y}$ Using LLL}

$\texttt{Solve}_{x,y}$ can also be regarded as a modular knapsack problem:

$$W=FA+GB=F\sum_{i=0}^{k-1}2^iA_i+G\sum_{i=0}^{k-1}2^iB_i=\sum_{i=0}^{2k-1} x_i c_i \bmod p$$

where:

\begin{equation*}
x_i=\begin{cases}
A_i & \text{if $0\leq i\leq k-1$}\\
B_{i-k} & \text{if $k\leq i\leq 2k-1$}
\end{cases}~~~~
c_i=\begin{cases}
2^i F~~~\bmod p& \text{if $0\leq i\leq k-1$}\\
2^{i-k}G \bmod p& \text{if $k\leq i\leq 2k-1$}
\end{cases}
\end{equation*}

However, if its density is too low, there is an efficient reduction to the problem of finding the shortest vector from Lenstra-Lenstra-Lovász's Algorithm (LLL, \cite{Lenstra82factoringpolynomials}). LLL gives a $(2/\sqrt{3})^n$ approximation ratio, where $n$ is the dimension of the lattice.

 We refer the reader to \cite{LLL} for more details and focus here on using LLL to solve the modular knapsack:

$$W=\sum_{i=0}^{k-1} x_i c_i \bmod p\mbox{~where~}c_i\in\{0,1\}$$




\begin{definition}[Modular Knapsack(or subset sum) Problem]
Let $B=\{c_0,...,c_{k-1}\}$ be a set of positive integers. Let $W=\sum_{i=0}^{k-1} x_i c_i \bmod p$, where $x_i \in \{0,1\}$.

A modular Knapsack problem is given $\{c_i\},p,W$, find each $x_i$.

$$W=\sum_{i=0}^{k-1} x_i c_i \bmod p\mbox{~where~}x_i\in\{0,1\}$$

\end{definition}



==> schemes.tex <==
\begin{center}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.8cm, semithick]
\tikzstyle{every state}=[fill=none,draw=black,text=black]

  \node[state,minimum width=5em,rectangle]         (A)              {RNG};
  \node[state,minimum width=5em,rectangle]         (B) [right of=A] {$\mathcal{H}(\alpha,m)$};
  \node[state,minimum width=5em,rectangle]         (C) [right of=B] {$\mathcal{H}'(A,B)$};
  \node[state,minimum width=5em,rectangle]         (D) [right of=C] {$\mathcal{F}_k(\alpha,m)$};
  \node at ($(A)!0.5!(B)$) (Q){};
  \node at ($(C)!0.5!(B)$) (P){};
  \node at ($(C)!0.5!(D)$) (L){};
  \node[state,minimum width=5em,rectangle]         (E) [above of=P,node distance=1.5cm] {$HA+B$};
  \coordinate[right of=D,node distance=1.8cm] (res0);
  \coordinate[above of=E,node distance=1.2cm] (res1);
  \coordinate[right of=E,node distance=1.8cm] (placeH);
  \coordinate[above of=D,node distance=1.2cm] (placeM);
  \coordinate[above of=B,node distance=1.2cm] (placeM2);
  \coordinate[below of=Q,node distance=1cm] (G);
  \coordinate[below of=D,node distance=1cm] (H);
  \coordinate[above of=P,node distance=1.5cm] (Z);
  \coordinate[above of=L,node distance=1.5cm] (T);
  \path (A) edge              node {$\alpha$} (B);
  \path (B) edge              node[below] {$A,B$} (C);
  \path (C) edge              node {$k$} (D);
  \draw[<-] (D.north)--(placeM) node[label={[yshift=-0.2cm]$m$}] {};
  \draw[<-] (B.north)--(placeM2) node[label={[yshift=-0.2cm]$m$}] {};  
  \draw[->] (D.east)--(res0) node {$~~~~C'$};
  \draw[->] (E.north)--(res1) node[label={[yshift=-0.2cm]$C$}] {};
  \draw[<-] (E.east)--(placeH) node {$~~~H$};
  \fill ($ (A) !.5! (B) $) circle [radius=2pt];
  \fill ($ (C) !.5! (B) $) circle [radius=2pt];
  \draw[->,rounded corners=.25cm] (Q.center) -- (G) -- (H) -- (D.south);
  \draw[->,rounded corners=.25cm] (P.center) -- (E.south);
\end{tikzpicture}
\end{center}

\begin{center}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.8cm, semithick]
\tikzstyle{every state}=[fill=none,draw=black,text=black]
  \node[state,minimum width=5em,rectangle]         (A) {$\sol_{x,y}$};
  \node[state,minimum width=5em,rectangle]         (B) [right of=A] {$\mathcal{H}'(A,B)$};
  \node[state,minimum width=5em,rectangle]         (C) [right of=B] {$\mathcal{F}^{-1}_k(C')$};
%  \node[state,minimum width=5em,rectangle]         (D) [right of=C] {};
  \node at ($(A)!0.5!(B)$) (Q){};
  \node at ($(C)!0.5!(D)$) (alphm){};
   \node[state,minimum width=5em,rectangle]        (X) [below of=P,node distance=1.5cm] {~$m$ valid if $(A,B)=\mathcal{H}(\alpha,m)$~~};
  \coordinate[right of=C,node distance=2.8cm] (D);
  \coordinate[above of=C,node distance=1.2cm] (placec0);  
  \coordinate[below of=A,node distance=1.5cm] (placec1);  
  \coordinate[below of=Q,node distance=1.5cm] (G);
  \coordinate[below of=alphm,node distance=1.5cm] (H);
  \path (A) edge node {$A,B$} (B);
  \path (B) edge node {$k$} (C);
  \path (C) edge node {$\alpha,m$} (D);
  \draw[<-] (C.north)--(placec0) node[label={[yshift=-0.2cm]$C'$}] {};
  \draw[<-] (A.south)--(placec1) node[label={[yshift=-0.65cm]$F,G,C$}] {};
  \fill ($ (A) !.5! (B) $) circle [radius=2pt];
  \fill ($ (C) !.5! (D) $) circle [radius=2pt];
  \draw[->,rounded corners=.25cm] (Q.center) -- (G) -- (X.west);
  \draw[<-,rounded corners=.25cm] (X.east) -- (H) -- (alphm.center);
\end{tikzpicture}
\end{center}
